Rethinking Memory in LLM based Agents: Representations, Operations, and Emerging Topics

Memory is fundamental to large language model (LLM)-based agents, but existing surveys emphasize application-level use (e.g., personalized dialogue), while overlooking the atomic operations governing memory dynamics. This work categorizes memory into parametric (implicit in model weights) and contextual (explicit external data, structured/unstructured) forms, and defines six core operations: Consolidation, Updating, Indexing, Forgetting, Retrieval, and Condensation. Mapping these dimensions reveals four key research topics: long-term, long-context, parametric modification, and multi-source memory. The taxonomy provides a structured view of memory-related research, benchmarks, and tools, clarifying functional interactions in LLM-based agents and guiding future advancements. The datasets, papers, and tools are publicly available at https://github.com/Elvin-Yiming-Du/Survey_Memory_in_AI.

==> tables/datasets-long-context-evaluation.tex <==
\begin{table*}[htbp]
\centering
% \small
%\rowcolors{2}{LC}{white}
\arrayrulecolor{black}
\resizebox{\textwidth}{!}{
\begin{tabular}{
    >{\arraybackslash}m{3cm}
    >{\arraybackslash}m{2.5cm}
    >{\arraybackslash}m{2.5cm}
    >{\arraybackslash}m{3.1cm}
    >{\arraybackslash}m{6.5cm}
    >{\arraybackslash}m{1.3cm}
}
\toprule
\textbf{Datasets} & \textbf{Modality} & \textbf{Operations} & \textbf{Metrics} & \textbf{Purpose} & \textbf{Year} \\
\midrule
\textbf{LongBench v2} \newline \citep{bai2025longbenchv2deeperunderstanding} & text + table + KG & compression, retrieval & Accuracy & Updated version of LongBench with longer and more challenging tasks in a consistent multiple-choice format for reliable evaluation. & 2024 \\

\textbf{SWE-bench Multimodal} \newline \citep{yang2025swebench} & text + image & compression, retrieval & Resolution rate, Inference cost & Extension of SWE-bench with multimodal data (517 task instances) to evaluate long-context reasoning with images. & 2024 \\

\textbf{$\infty$Bench} \newline \citep{zhang-etal-2024-bench} & text & compression, retrieval & F1, Accuracy, ROUGE-L-Sum & Benchmark with 12 sub-tasks targeting \textbf{extreme long context} (average context surpassing 100K tokens). & 2024 \\

\textbf{L-Eval} \newline \citep{an-etal-2024-l} & text & compression, retrieval & ROUGE-L, F1, GPT4 & Contains 20 sub-tasks specifically designed for evaluating long-context language models from multiple perspectives. & 2023 \\

\textbf{LongBench} \newline \citep{bai-etal-2024-longbench} & text & compression, retrieval & F1, ROUGE-L, Accuracy, EM, Edit Sim & Includes 14 English tasks, 5 Chinese tasks, and 2 code tasks for systematic long-context evaluation. & 2023 \\

\textbf{SWE-bench} \newline \citep{jimenez2024swebench} & text & compression, retrieval & Resolution rate (\% Resolved) & Evaluates LLMs' ability to solve real GitHub issues (2,294 instances) requiring reasoning over large codebases. & 2023 \\

\textbf{LooGLE} \newline \citep{li-etal-2024-loogle} & text & compression, retrieval & BLEU-1, BLEU-4, ROUGE-1, ROUGE-4, ROUGE-L, Meteor, Bert, GPT-4 scores & Benchmark with 7 tasks designed for \textbf{extreme long context} (documents exceeding 24K tokens). & 2023 \\

\textbf{GovReport} \newline \citep{huang-etal-2021-efficient} & text & compression & ROUGE-1, ROUGE-2, ROUGE-L, Bert Score & Reports from government agencies for evaluating long-document summarization. & 2021 \\

\textbf{MusiQue} \newline \citep{trivedi-etal-2022-musique} & text & retrieval & F1 & Multi-hop QA dataset for evaluating long-context reasoning and QA ability. & 2021 \\

\textbf{LRA} \newline \citep{tay2021long} & text + image & compression, retrieval & Accuracy & Benchmark with six tasks for evaluating efficient long-context modeling. & 2020 \\

\textbf{NaturalQuestions} \newline \citep{kwiatkowski2019natural} & text & retrieval & EM, F1 & QA dataset for testing reasoning and retrieval with long contexts. & 2019 \\

\textbf{PG-19} \newline \citep{Rae2020Compressive} & text & compression & PPL & Corpus of long books from Project Gutenberg for language modeling with long contexts. & 2019 \\

\textbf{TriviaQA} \newline \citep{joshi-etal-2017-triviaqa} & text & retrieval & EM, F1 & QA dataset suitable for evaluating long-context understanding and reasoning. & 2017 \\

\textbf{NarrativeQA} \newline \citep{kocisky-etal-2018-narrativeqa} & text & retrieval & BLEU-1, BLEU-4, Meteor, ROUGE-L, MRR & QA dataset designed to evaluate comprehension over narrative text with long contexts. & 2017 \\

\textbf{CNN/DailyMail} \newline \citep{nallapati-etal-2016-abstractive} & text & compression & ROUGE-1, ROUGE-2, ROUGE-L & Dataset of 300k news articles for long-document summarization tasks. & 2016 \\

\textbf{WikiText-103} \newline \citep{merity2017pointer} & text & compression & PPL & Corpus of 100 million tokens from verified Wikipedia articles for long-context language modeling. & 2016 \\
\bottomrule
\end{tabular}
}
\caption{Datasets for \textbf{long-context memory} evaluation.}
\label{tab:longcontext_dataset}
\end{table*}


==> tables/methods-long-context-contextual-utilization.tex <==
\begin{table*}[t!]
\centering
% \small
% \rowcolors{2}{LC}{white}
\arrayrulecolor{black}
\resizebox{\textwidth}{!}{
\begin{tabular}{
    >{\raggedright\arraybackslash}m{2.5cm}
    >{\raggedright\arraybackslash}m{2cm}
    >{\raggedright\arraybackslash}m{1cm}
    >{\raggedright\arraybackslash}m{1cm}
    >{\raggedright\arraybackslash}m{2cm}
    >{\raggedright\arraybackslash}m{4cm}
    >{\raggedright\arraybackslash}m{5cm}
    >{\raggedright\arraybackslash}m{1cm}
}
\toprule
\textbf{Method} & \textbf{Type} & \textbf{SM} & \textbf{TM} & \textbf{Operations} & \textbf{LMs} & \textbf{Features} & \textbf{Year} \\
\toprule
\textbf{Sparse RAG} \newline \citep{zhu2025accelerating} 
& Context Selection 
& T & P 
& Retrieval 
& Gemini 
& Sparse context selection, reduces the number of documents involved during decoding 
& 2025 \\

\textbf{GraphReader} \newline \citep{li-etal-2024-graphreader} 
& Context Selection 
& T & G 
& Retrieval 
& GPT-4-128k 
& Graph-based agent; structures long context into a graph 
& 2024 \\

\textbf{Ziya-Reader} \newline \citep{he-etal-2024-never} 
& Context Selection 
& T & T 
& Retrieval 
& Ziya2-13B-Base (LLaMA-2-13B) 
& Supervised fine-tuning; position-agnostic multi-step QA 
& 2024 \\

\textbf{FILM} \newline \citep{NEURIPS2024_71c3451f} 
& Context Selection 
& T & T 
& Retrieval 
& FILM-7B (Mistral 7B) 
& Data-driven approach; addresses the “lost in the middle” problem 
& 2024 \\

\textbf{RECOMP} \newline \citep{xu2024recomp} 
& Context Compression 
& T & T 
& Compression 
& GPT-2, GPT2-XL, GPT-J, Flan-UL2 
& Hard prompt compression with extractive and abstractive strategies 
& 2024 \\

\textbf{LongLLMLingua} \newline \citep{jiang-etal-2024-longllmlingua} 
& Context Compression 
& T & T 
& Compression 
& GPT-3.5-Turbo-06136, LongChat-13B-16k 
& Hard prompt compression for efficient input representation 
& 2024 \\

\textbf{LLMLingua-2} \newline \citep{pan-etal-2024-llmlingua} 
& Context Compression 
& T & T 
& Compression 
& XLM-RoBERTa-Large, Multilingual-BERT 
& Hard prompt compression with data distillation for multilingual contexts 
& 2024 \\

\textbf{QGC} \newline \citep{cao-etal-2024-retaining} 
& Context Compression 
& T & T 
& Compression 
& LongChat-13B-16K, LLaMA-2-7B 
& Query-guided dynamic context compression 
& 2024 \\

\textbf{xRAG} \newline \citep{cheng2024xrag} 
& Context Compression 
& T & P 
& Compression 
& Mistral-7B, Mixtral-8x7B 
& Soft prompt compression for parametric integration 
& 2024 \\ 

\textbf{AutoCompressor} \newline \citep{chevalier-etal-2023-adapting} 
& Context Compression 
& T & P 
& Compression 
& OPT-1.3B, OPT-2.7B, LLaMA-2-7B 
& Soft prompt compression for general-purpose efficiency 
& 2023 \\
\bottomrule
\end{tabular}
}
\caption{Overview of methods for \textbf{long-context memory in contextual utilization}. ``SM'' (Source Modality) denotes the source modality of contextual memory. ``TM'' (Target Modality) denotes the target modality (processed for selection or after compression): T – Text, G – Graphs, P – Parametric.}
\label{tab:Cha-longcontexteffectiveness}
\end{table*}


==> tables/methods-long-context-efficiency.tex <==
\begin{table*}[t!]
\centering
%\small
%\rowcolors{2}{LC}{white}
\arrayrulecolor{black}
\resizebox{\textwidth}{!}{
\begin{tabular}{
    >{\raggedright\arraybackslash}m{2.5cm}
    >{\raggedright\arraybackslash}m{2cm}
    >{\raggedright\arraybackslash}m{1cm}
    >{\raggedright\arraybackslash}m{1cm}
    >{\raggedright\arraybackslash}m{2cm}
    >{\raggedright\arraybackslash}m{4cm}
    >{\raggedright\arraybackslash}m{5cm}
    >{\raggedright\arraybackslash}m{1cm}
}
\toprule
 \textbf{Method} & \textbf{Type} & \textbf{TF} & \textbf{DF} & \textbf{Operations} & \textbf{LMs} & \textbf{Features} & \textbf{Year} \\
\toprule 
 \textbf{TokenSelect} \newline \citep{wu2025tokenselectefficientlongcontextinference} 
 & KV Cache Selection 
 & \usym{2713} 
 & \usym{2713} 
 & Retrieval 
 & Qwen2 7B, Llama-3 8B, Yi-1.5-6B 
 & Dynamic token-level KV cache selection 
 & 2025 \\

 \textbf{StreamingLLM} \newline \citep{xiao2024efficient} 
 & KV Cache Dropping 
 & \usym{2713} 
 & \usym{2717} 
 & Compression 
 & Llama-2, MPT, PyThia, Falcon 
 & Static KV cache dropping, Attention sink in the initial tokens 
 & 2024 \\

 \textbf{FastGen} \newline \citep{ge2024model} 
 & KV Cache Dropping 
 & \usym{2713} 
 & \usym{2717} 
 & Compression 
 & Llama-1 7B/13B/30B/65B 
 & Adaptive profiling-based KV cache dropping 
 & 2024 \\

 \textbf{SnapKV} \newline \citep{NEURIPS2024_28ab4182} 
 & KV Cache Dropping 
 & \usym{2713} 
 & \usym{2717} 
 & Compression 
 & LWM-Text-Chat-1M, LongChat-7b-v1.5-32k, Mistral-7B-Instruct-v0.2, Mixtral-8x7B-Instruct-v0.1 
 & Head-wise KV cache dropping, Attention head behavior 
 & 2024 \\

 \textbf{LESS} \newline \citep{pmlr-v235-dong24f} 
 & KV Cache Storing Optimization 
 & \usym{2717} 
 & \usym{2713} 
 & Compression 
 & Llama-2 13B, Falcon 7B 
 & Low-rank KV cache storage enabling querying of all tokens 
 & 2024 \\

 \textbf{KIVI} \newline \citep{pmlr-v235-liu24bz} 
 & KV Cache Storing Optimization 
 & \usym{2713} 
 & \usym{2713} 
 & Compression 
 & Llama-2 7B/13B, Llama-3 8B, Falcon 7B, Mistral-7B 
 & Asymmetrical KV cache quantization 
 & 2024 \\

 \textbf{KVQuant} \newline \citep{NEURIPS2024_028fcbcf} 
 & KV Cache Storing Optimization 
 & \usym{2713} 
 & \usym{2713} 
 & Compression 
 & LLaMA-7B/13B/30B/65B, Llama-2-7B/13B/70B, Llama-3-8B/70B, Mistral-7B 
 & KV cache quantization 
 & 2024 \\

 \textbf{QUEST} \newline \citep{pmlr-v235-tang24l} 
 & KV Cache Selection 
 & \usym{2713} 
 & \usym{2713} 
 & Retrieval 
 & LongChat-7B-v1.5-32K, Yarn-Llama2-7B-128K 
 & Query-aware KV cache selection 
 & 2024 \\

 \textbf{H$_2$O} \newline \citep{zhang2023ho} 
 & KV Cache Dropping 
 & \usym{2713} 
 & \usym{2717} 
 & Compression 
 & OPT, Llama-1, GPT-NeoX 
 & Dynamic KV cache dropping, Retain Heavy Hitter tokens 
 & 2023 \\

 \textbf{Scissorhands} \newline \citep{liu2023scissorhands} 
 & KV Cache Dropping 
 & \usym{2713} 
 & \usym{2717} 
 & Compression 
 & OPT 6.7B, 13B, 30B, 66B 
 & Dynamic KV cache dropping, Persistence of importance hypothesis 
 & 2023 \\

 \textbf{FlexGen} \newline \citep{10.5555/3618408.3619696} 
 & KV Cache Storing Optimization 
 & \usym{2713} 
 & \usym{2713} 
 & Compression 
 & OPT 6.7B to 175B 
 & KV cache quantization and offloading 
 & 2023 \\

 \textbf{Memorizing Transformers} \newline \cite{wu2022memorizing} 
 & KV Cache Selection 
 & \usym{2717} 
 & \usym{2713} 
 & Retrieval 
 & Transformers 
 & External KV cache memory for enhanced recall 
 & 2022 \\
\bottomrule
\end{tabular}
}
\caption{Overview of methods for \textbf{long-context memory in parametric efficiency}. ``TF'' (Training Free) indicates no additional gradient-based updates. ``DF'' (Dropping Free) indicates that the method preserves all KV cache without dropping.}
\label{tab:Cha-longcontextefficiency}
\end{table*}


==> tables/methods-multi-modal.tex <==
\begin{table*}[t!]
\centering
%\small
%\rowcolors{2}{MS}{white}
\arrayrulecolor{black}
\resizebox{\textwidth}{!}{
\begin{tabular}{
    >{\raggedright\arraybackslash}m{2cm}
    >{\raggedright\arraybackslash}m{1.7142cm}
    >{\raggedright\arraybackslash}m{0.8571cm}
    >{\raggedright\arraybackslash}m{0.8571cm}
    >{\raggedright\arraybackslash}m{1.7142cm}
    >{\raggedright\arraybackslash}m{1.2856cm}
    >{\raggedright\arraybackslash}m{1.2856cm}
    >{\raggedright\arraybackslash}m{1.7142cm}
    >{\raggedright\arraybackslash}m{1.7142cm}
    >{\raggedright\arraybackslash}m{3.4284cm}
    >{\raggedright\arraybackslash}m{0.8571cm}
}
\toprule
 \textbf{Method} & \textbf{Type} & \textbf{TF} & \textbf{DS} & \textbf{Mo} & \textbf{Input} & \textbf{Output} & \textbf{Modeling} & \textbf{Ops} & \textbf{Features}  & \textbf{Year} \\
\toprule

\textbf{IGSR}\newline\cite{wang2025new} & retrieval & \usym{2713} & \usym{2713} & text + image & image-text dialogue & stickers & LLaVa, GPT4, Qwen-VL, CLIP, Llama3 & retrieval & multi-modal memory bank, sticker retrieval, intention aware cross-session dialogue & 2025 \\

\textbf{VISTA}\newline\cite{zhou2024vista} & retrieval & \usym{2713} & \usym{2717} & text + image & image-text query & retrieved response & CLIP, BLIP-B, Pic2Word & retrieval & Visual Token Injection, composed data fine-tuning & 2024 \\

\textbf{UniVL-DR} \newline\cite{liu2023univldr} & retrieval & \usym{2717} & \usym{2717} & text + image & image-text query & retrieved response & VinVLDPR, CLIP-DPR & retrieval & Modality-balanced hard negatives & 2023 \\

\textbf{MultiInstruct*} \newline\cite{xu-etal-2023-multiinstruct} & fusion & \usym{2713} & \usym{2717} & text + image & instruction + instances & response & OFA & compression & Cross-modal transfer learning & 2023 \\

\textbf{NextChat} \newline\cite{zhang2023nextchat} & fusion & \usym{2717} & \usym{2713} & text + image + boxes & image + text & response & CLIP & compression & Cross-modal alignment & 2023 \\

\textbf{UniTranSeR}\newline\cite{ma-etal-2022-unitranser} & fusion & \usym{2717} & \usym{2713} & text + image & context & response & MLM + MPM & compression & Intention-aware response generation, unified transformer space & 2022 \\

\bottomrule
\end{tabular}
}
\caption{Overview of methods for \textbf{multi-source memory in Multi-modal Coordination}. "TF" (Training Free) denotes whether the method operates without additional gradient-based updates. "DS" (Dialogue System) denotes whether the method aims for a dialogue task. "Mo" denotes data modality (T – Text, I – Images, B – Box (Position)).}
\label{tab:Cha-multi_modal_multi_source}
\end{table*}

